Probabilistic Asynchronous Arbitrary Pattern Formation

We propose a new probabilistic pattern formation algorithm for oblivious mobile robots that operates inthe ASYNC model. Unlike previous work, our algorithm makes no assumptions about the local coordinatesystems of robots (the robots do not share a common "North" nor a common "Right"), yet it preserves theability from any initial configuration that contains at least 5 robots to form any general pattern (and not justpatterns that satisfy symmetricity predicates). Our proposal also gets rid of the previous assumption (in thesame model) that robots do not pause while moving (so, our robots really are fully asynchronous), and theamount of randomness is kept low -- a single random bit per robot per Look-Compute-Move cycle is used.Our protocol consists in the combination of two phases, a probabilistic leader election phase, and a deterministicpattern formation one. As the deterministic phase does not use chirality, it may be of independentinterest in the deterministic context. A noteworthy feature of our algorithm is the ability to form patternswith multiplicity points (except the gathering case due to impossibility results), a new feature in the contextof pattern formation that we believe is an important asset of our approach.

==> fig_angle_of_robots_less_than_the_shift.tex <==
%!TEX root = async_pattern_formation.tex
\begin{figure}\centering
\begin{tikzpicture}[line cap=round,line join=round,>=triangle 45,x=1.0cm,y=1.0cm, scale=0.8]
%\clip(-1.6433983163585213,-11.418927044133492) rectangle (11.440361359849675,3.1451120114997337);
\draw [shift={(4.96724,-3.120403248434688)},color=black,fill=black,fill opacity=0.1] (0,0) -- (0.05424462911987458:0.7162642158508136) arc (0.05424462911987458:45.05424462911988:0.7162642158508136) -- cycle;
\draw [shift={(4.96724,-3.120403248434688)},color=black,fill=black,fill opacity=0.1] (0,0) -- (45.05424462911987:0.7162642158508136) arc (45.05424462911987:81.90659576669549:0.7162642158508136) -- cycle;
\draw [shift={(5.770936899769914,2.531329487714625)},color=black,fill=black,fill opacity=0.1] (0,0) -- (-134.94575537088014:0.7162642158508136) arc (-134.94575537088014:-98.09340423330453:0.7162642158508136) -- cycle;
\draw [shift={(0.12532016650254896,-3.124987324719216)},color=black,fill=black,fill opacity=0.1] (0,0) -- (0.054244629119876785:0.7162642158508136) arc (0.054244629119876785:45.05424462911987:0.7162642158508136) -- cycle;
\draw [shift={(2.549338084692249,-6.352702142678828)},color=black,fill=black,fill opacity=0.1] (0,0) -- (53.201893491544254:0.7162642158508136) arc (53.201893491544254:90.05424462911986:0.7162642158508136) -- cycle;
\draw(4.96724,-3.120403248434688) circle (5.70859103698641cm);
\draw (4.96724,-3.120403248434688)-- (9.,0.92);
\draw (0.12532016650254896,-3.124987324719216)-- (5.770936899769914,2.531329487714625);
\draw (5.770936899769914,2.531329487714625)-- (4.96724,-3.120403248434688);
\draw(2.5469501179204053,-3.8304178357294814) circle (2.522285437350074cm);
\draw (0.12532016650254896,-3.124987324719216)-- (2.549338084692249,-6.352702142678828);
\draw (2.549338084692249,-6.352702142678828)-- (4.96724,-3.120403248434688);
\draw (5.232738155809289,-1.8867299176688658) node[anchor=north west, opacity=0, text opacity=1] {$\theta$};
\draw (5.807757110277041,-2.4538582347007225) node[anchor=north west, opacity=0, text opacity=1] {$\frac{\pi}{4}$};
\draw (0.806156651597958,-2.4538582347007225) node[anchor=north west, opacity=0, text opacity=1] {$\frac{\pi}{4}$};
\draw (5.041734364915739,1.4900930570319814) node[anchor=north west, opacity=0, text opacity=1] {$\theta$};
\draw (2.6780624526080543,-5.1860434151358366) node[anchor=north west, opacity=0, text opacity=1] {$\theta$};
\draw (10.675828478594184,-3.12)-- (-0.7413484785941832,-3.12);
\draw (2.544562151148561,-1.3081335287801341)-- (2.549338084692249,-6.352702142678828);
\begin{scriptsize}
\draw [fill=black] (9.,0.92) circle (1.5pt);
\draw [fill=black] (4.96724,-3.120403248434688) circle (1.5pt);
\draw[color=black, opacity=0, text opacity=1] (5.662496685319777,-3.5877716174979213) node {$W(P)$};
\draw [fill=black] (9.76724,-3.120403248434688) circle (1.5pt);
\draw[color=black, opacity=0, text opacity=1] (9.662496685319777,-3.5877716174979213) node {$w$};
\draw [fill=black] (4.96724,-3.124987324719216) circle (1.5pt);
\draw[color=black, opacity=0, text opacity=1] (-0.18,-2.6133752937216998) node {$W(P')$};
\draw [fill=black] (5.770936899769914,2.531329487714625) circle (1.5pt);
\draw[color=black, opacity=0, text opacity=1] (6.0206287932451845,2.1184666354468997) node {$r'$};
\draw [fill=black] (2.5469501179204053,-3.8304178357294814) circle (1.5pt);
\draw[color=black, opacity=0, text opacity=1] (9.0206287932451845,1.1184666354468997) node {$r$};
\draw [fill=black] (2.549338084692249,-6.352702142678828) circle (1.5pt);
\draw[color=black, opacity=0, text opacity=1] (3.1078209821185423,-6.572205850209647) node {$F$};
\draw [fill=black] (2.544562151148561,-1.3081335287801341) circle (1.5pt);
\draw[color=black, opacity=0, text opacity=1] (2.7019379264697476,-0.9853449665732956) node {$H$};
\draw [fill=black] (2.5462800832512746,-3.122695286576952) circle (1.5pt);
\draw[color=black, opacity=0, text opacity=1] (2.7019379264697476,-2.7998809800620252) node {$B$};
\end{scriptsize}
\end{tikzpicture}
\caption{Worst case for the angle $ang_{\min}(W(P),p,W(P'))$}\label{fig: Worst case for the angle ang_min(W(P),p,W(P'))}
\end{figure}

==> fig_notations.tex <==
%!TEX root = async_pattern_formation.tex

\tikzstyle{every node}=[circle, draw, fill=black!50,%
                        inner sep=0pt, minimum width=4pt]
\begin{figure}
\centering
\begin{subfigure}[b]{0.48\textwidth}
\caption{A configuration}
\begin{tikzpicture}[every path/.style={>=stealth}]


\draw (35:2.1) node[opacity=0, text opacity=1] {$C(P)$};
\draw[dashed] (0:0) circle (1.6);
\draw (0:0) node[fill=white,label={90:$c(P)$}] {};

\draw (0:1.6) node {};
\draw (90:1.6) node {};
\draw (180:1.1) node {};
\draw (-30:0.8) node {};

\draw (-10:0.5) node[opacity=0, text opacity=1] {$l_P$};
\draw[<->] (-30:0.08) -- (-30:0.73);
\draw (0+30:1.4) node {};
\draw (90+30:1.2) node {};
\draw (180+30:0.4) node {};
\draw (-110:1.6) node {};



\end{tikzpicture}
\end{subfigure}
\end{figure}

==> fig_regular_set.tex <==
%!TEX root = opodis.tex

\tikzstyle{every node}=[circle, draw, fill=black!50,%
                        inner sep=0pt, minimum width=4pt]
\begin{figure}
\centering
%\begin{subfigure}[b]{0.20\textwidth}\centering
\subfloat[A configuration of robots that contains a selected robot and the pattern to form (white nodes)]{
\begin{tikzpicture}[every path/.style={>=stealth}, scale=0.7]
 
{ [pattern color=black!50]
\draw[color=black!50, pattern=north east lines] (0:0) circle (0.6) {};
}
\draw[color=black!50,fill=white] (0:0) circle (0.3) {};

\draw[] (-45:1.9) node[rectangle,opacity=0, text opacity=1] {\scriptsize $C(P)=C(F)$};
\draw[dashed] (-35:1.8) arc (-35:295:1.8);
\draw[fill=black] (0:0) circle (0.04) {};

\draw (0:1.8) node {};
\draw (90:1.8) node {};
\draw (160:0.7) node {};

\draw (0:0.8) node[opacity=0, text opacity=1] {$l_F$};
\draw[<->] (-30:0.08) -- (-30:0.83);
\draw (0+30:1.6) node {};
\draw (90+30:1.4) node {};
\draw (180+30:0.3) node {};
\draw (-110:1.8) node {};


\tikzstyle{fakeNode}=[circle, draw=black, fill=white]
\draw (0+00:1.6) node[fakeNode] {};
\draw (90+10:0.4) node[fakeNode] {};
\draw (-30:0.9) node[fakeNode] {};
\draw (-180:1.8) node[fakeNode] {};
\draw (-180:1.8) node[fakeNode] {};
\draw (-90:1.8) node[fakeNode] {};
\draw (60:1.8) node[fakeNode] {};

\end{tikzpicture}
%\phantomsubcaption
%\vspace{-0.29cm}
\label{fig:a configuration that contains a selected robot}%
}
%\end{subfigure}
%\begin{subfigure}[b]{0.23\textwidth}\centering
~
\subfloat[a $5$-regular set]{
\begin{tikzpicture}[every path/.style={>=stealth}, scale=0.7]

\tikzstyle{fakeNode}=[circle, draw=black, fill=white]
%\draw (0:0) node {};
\draw[] (0:0) -- (0:1.9);
\draw[] (0:0) -- (0+360/5:1.9);
\draw[] (0:0) -- (0+2*360/5:1.9);
\draw[] (0:0) -- (0+3*360/5:1.9);
\draw[] (0:0) -- (0+4*360/5:1.9);

\draw[] (0:1.2) node {};
\draw[] (0+360/5:1.7) node {};
\draw[] (0+2*360/5:1.0) node {};
\draw[] (0+3*360/5:0.5) node {};
\draw[] (0+4*360/5:1.6) node {};

\draw (0:1.0) arc (0:360/5:1.0);
\draw (36:1.5) node[text opacity=1,opacity=0] {$\alpha$};


\end{tikzpicture}
%\phantomsubcaption
\label{fig:a 5-regular set}
}~%\end{subfigure}
\subfloat[a bi-angled $4$-regular set]{
%\begin{subfigure}[b]{0.23\textwidth}\centering
\begin{tikzpicture}[scale=0.7]

%\draw (0:0) node {};
\draw[] (0:2.1) -- (180:1.9);
\draw[] (90:2.0) -- (-90:1.8);

\draw (0:1.6) node {};
\draw (90:1.6) node {};
\draw (180:1.5) node {};
\draw (-90:1.1) node {};

\draw[] (0+30:2.1) -- (180+30:1.9);
\draw[] (90+30:1.9) -- (-90+30:1.9);

\draw (0+30:1.4) node {};
\draw (90+30:1.2) node {};
\draw (180+30:1.1) node {};
\draw (-90+30:1.6) node {};


\tikzstyle{virtualAxis} = [dashed, red!90]
\draw[virtualAxis] (0+15:1.9) -- (180+15:1.9);
\draw[virtualAxis] (90+15:1.9) -- (-90+15:1.9);
\draw[virtualAxis] (0-30:1.9) -- (180-30:1.9);
\draw[virtualAxis] (90-30:1.9) -- (-90-30:1.9);

\draw (0:1.9) arc (0:30:1.9);
\draw (15:2.2) node[text opacity=1,opacity=0] {$\alpha$};
\draw (30:1.9) arc (30:90:1.9);
\draw (50:2.2) node[text opacity=1,opacity=0] {$\beta$};

\end{tikzpicture}
%\phantomsubcaption
\label{fig:a bi-angled regular set}
%\end{subfigure}
}~
%\begin{subfigure}[b]{0.32\textwidth}\centering
\subfloat[a bi-angled shifted-$4$-regular set]{
\begin{tikzpicture}[every path/.style={>=stealth}, scale=0.7]

\tikzstyle{fakeNode}=[circle, draw=black, fill=white]
%\draw (0:0) node {};
\draw[] (0:2.1) -- (180:1.9);
\draw[] (90:1.9) -- (-90:1.7);

\draw[dashed] (0:0) circle (1.1);

\draw (10:1.1) node {};
\draw (90:1.6) node {};
\draw (180:1.5) node {};
\draw (0:1.1) node[fakeNode] {};
\draw (-90:1.4) node {};

\draw[] (0+30:1.9) -- (180+30:1.9);
\draw[] (90+30:1.9) -- (-90+30:1.9);

\draw (0+30:1.9) node {};
\draw (90+30:1.2) node {};
\draw (180+30:1.4) node {};
\draw (-90+30:1.6) node {};


\draw[red!90] (0,0) -- (10:2.1);
\draw[<->] (0:2.1) arc (0:10:2.1);
\draw (4:3.3) node[text opacity=1,opacity=0] {$<\alpha_{\min}/4$};

%\draw[virtualAxis] (0+15:2.1) -- (180+15:2.1);
%\draw[virtualAxis] (90+15:2.1) -- (-90+15:2.1);
%\draw[virtualAxis] (0-30:2.1) -- (180-30:2.1);
%\draw[virtualAxis] (90-30:2.1) -- (-90-30:2.1);

\end{tikzpicture}
%\phantomsubcaption
\label{fig:a bi-angled shifted 4-regular set}
%\end{subfigure}
}
\caption{Examples of configurations}

\end{figure}


\begin{figure}\centering
%\begin{subfigure}[b]{0.31\textwidth}\centering
\subfloat[nA configuration that strictly contains a bi-angled $2$-regular set. $2=\rho(P\backslash reg(P))$ and the virtual axis of $reg(P)$ are axis of symmetry of $P\backslash reg(P)$.]{
\begin{tikzpicture}[scale=0.9]

%\draw (0:0) node {};
\draw[] (0-15:1.5) -- (180-15:1.4);

\draw (0-15:1.1) node {};
\draw (180-15:1.0) node {};

\draw[] (0+15:1.5) -- (180+15:1.4);

\draw (0+15:1.2) node {};
\draw (180+15:0.6) node {};

\tikzstyle{virtualAxis} = [dashed, red!90]
\draw[virtualAxis] (0:2.2) -- (180:2.2);
\draw[virtualAxis] (90:1.5) -- (90:0.7);
\draw[virtualAxis] (90:0.1) -- (-90:1.5);


\draw (25:1.85) node {};
\draw (38:1.95) node {};
\draw (-25:1.85) node {};
\draw (-38:1.95) node {};

\draw (180+25:1.85) node {};
\draw (180+38:1.95) node {};
\draw (180-25:1.85) node {};
\draw (180-38:1.95) node {};

\draw[dashed] (0+28:1.45) rectangle (180+28:1.35);
\draw (60:0.5) node[text opacity=1,opacity=0] {$reg(P)$};

%empty
%\draw (90:1.9) node[text opacity=1,opacity=0] {};

\end{tikzpicture}
%\caption{A configuration that strictly contains a bi-angled $2$-regular set. $2=\rho(P\backslash reg(P))$ and the virtual axis of $reg(P)$ are axis of symmetry of $P\backslash reg(P)$.}
%\end{subfigure}
}~~
%\begin{subfigure}[b]{0.31\textwidth}\centering
\subfloat[A configuration that strictly contains a $4$-regular set. We see that $4$ divides $8=\rho(P\backslash reg(P))$.]{
\begin{tikzpicture}[scale=0.9]

%\draw (0:0) node {};
\draw[] (0,0) -- (0:1.2);
\draw[] (0,0) -- (90:1.0);
\draw[] (0,0) -- (180:1.2);
\draw[] (0,0) -- (-90:1.0);

\draw[dashed] (12:1.9) -- (12+45:1.9) -- (12+90:1.9) -- (12+135:1.9) -- (12-180:1.9) -- (12-135:1.9) -- (12-90:1.9) -- (12-45:1.9) -- (12:1.9);

\draw (0:0.3) node {};
\draw (90:0.4) node {};
\draw (180:0.7) node {};
\draw (-90:0.5) node {};


\draw (12:1.9) node {};
\draw (12+45:1.9) node {};
\draw (12+90:1.9) node {};
\draw (12+135:1.9) node {};
\draw (12-180:1.9) node {};
\draw (12-135:1.9) node {};
\draw (12-90:1.9) node {};
\draw (12-45:1.9) node {};

%\draw[dashed] (-1,-0.7) rectangle (1,0.7);
\draw [dashed] plot [smooth cycle] coordinates {(-1.25,-0.7) (0.7,-0.7) (0.7,0.7) (-0.7,0.5)};
\draw (-0.7,-0.5) node[text opacity=1,opacity=0] {$reg(P)$};


\end{tikzpicture}
%\caption{A configuration that strictly contains a $4$-regular set. We see that $4$ divides $8=\rho(P\backslash reg(P))$.}
%\end{subfigure}
}
~~
\subfloat[$r_1$ and $r_1'$ have the greatest view but hold $C(P)$ so $reg(P)=\{r_2, r_2'\}$.]{
%\begin{subfigure}[b]{0.31\textwidth}\centering
\begin{tikzpicture}[scale=0.8]

%\draw (0:0) node {};
\tikzstyle{virtualAxis} = [dashed, red!90]
\draw[virtualAxis] (180:2) -- (0:2);


\draw (0, 0) circle (1.8);

\draw (5:1.8) node {};
\draw (-5:1.8) node {};
\draw (8:2.15) node[text opacity=1,opacity=0] {$r_1$};
\draw (-8:2.15) node[text opacity=1,opacity=0] {$r_1'$};

\draw (180-50:1.8) node {};
\draw (180-30:1.8) node {};
\draw (180-10:1.8) node {};
\draw (180+10:1.8) node {};
\draw (180+30:1.8) node {};
\draw (180+50:1.8) node {};

\draw (180-50:1.45) node[text opacity=1,opacity=0] {$r_2$};
\draw (180-30:1.45) node[text opacity=1,opacity=0] {$r_3$};
\draw (180-10:1.45) node[text opacity=1,opacity=0] {$r_4$};
\draw (180+10:1.45) node[text opacity=1,opacity=0] {$r_4'$};
\draw (180+30:1.45) node[text opacity=1,opacity=0] {$r_3'$};
\draw (180+50:1.45) node[text opacity=1,opacity=0] {$r_2'$};

%empty
%\draw (90:3) node[text opacity=1,opacity=0] {};



\end{tikzpicture}
%\caption{$r_1$ and $r_1'$ have the greatest view but hold $C(P)$ so $reg(P)=\{r_2, r_2'\}$.}
%\end{subfigure}
}
\caption{Examples of configurations that strictly contain a regular set.}
\end{figure}

==> introduction.tex <==
%!TEX root = opodis.tex
We consider a set of mobile robots that move freely in a continuous 2-dimensional Euclidian space. %The robots are identical, autonomous and cannot communicate explicitly.
Each robot repeats a Look-Compute-Move (LCM) cycle~\cite{Suzuki99}. First, it \emph{Looks} at its surroundings to obtain a snapshot containing the locations of all robots as points in the plane, with respect to its ego-centered coordinate system. Based on this visual information, the robot \emph{Computes} a destination and then \emph{Moves} towards the destination.
The robots are identical, anonymous and oblivious \ie, the computed destination in each cycle depends only on the snapshot obtained in the current
cycle (and not on the past history of execution). The snapshots obtained by the robots are not consistently oriented in any manner.

The literature defines three different models of execution: in the fully synchronous (FSYNC) model, robots execute LCM cycles in a lock-step manner, in the semi-synchronous (SSYNC) model, each LCM cycle is supposed atomic, %This is equivalent to say that each time instant, a subset of robots is activated and preform a cycle synchronously. 
and in the most general asynchronous (ASYNC) model, each phase of each LCM cycle may take an arbitrary amount of time. This last model enables the possibility that a robot observes another robot while the latter is moving (and moving robots appear in the snapshot \emph{exactly the same way static robots do}), and that move actions are based on obsolete observations.

In this particularly weak model it is interesting to characterize which additional assumptions are needed for the robots to cooperatively perform a given task. In this paper, we consider the pattern formation problem in the most general ASYNC model. The robots start in an arbitrary initial configuration where no two robots occupy the same position, and are given the pattern to be formed as a set of coordinates in their own local coordinate system. An algorithm solves the pattern formation problem is within finite time the robots form the input pattern and remain stationary thereafter.

\paragraph*{Related Works.}

The pattern formation problem has been extensively studied in the deterministic setting~\cite{bouzid2011pattern,BouzidDPT10,Yamashita2010,Yamashita2012,Shantanu2010,YamashitaS10,Yamauchi13,DieudonnePV10,Flocchini08,Suzuki99}. 
The seminal paper on mobile robots~\cite{Suzuki99} presents a deterministic solution to construct general patterns in the SSYNC model, with the added assumption that robots have access to an infinite non-volatile memory (that is, robots are \emph{not} oblivious). The construction was later refined for the ASYNC model by Bouzid \emph{et al.}, still using a finite number of infinite precision variables. 

The search for an oblivious solution to the general pattern formation proved difficult~\cite{Flocchini08}. For oblivious deterministic robots to be able to construct any general pattern, it is required that they agree on a common ``North'' (that is, a common direction and orientation) but also on a common ``Right'' (that is, a common chirality), so that robots get to all agree on a common coordinate system. If only a ``North'' (and implicitly if only a ``Right'') is available, then some patterns involving an even number of robots cannot be formed. 
Relaxing the common coordinate system condition let to a characterization of the patterns that can be formed by deterministic oblivious robots~\cite{Yamashita2010,Yamashita2012,Yamauchi13}. The best deterministic algorithm so far in the ASYNC model without a common coordinate system~\cite{Yamauchi13} proves the following: If $\rho$ denotes the geometric symmetricity of a robot configuration, and $I$ and $P$ denote the initial and target configurations, respectively, then $P$ can be formed if and only if $\rho(I)$ divides $\rho(F)$. All aforementioned deterministic solutions assume that both the input configurations and the target configuration do not have multiplicity points (that is, locations hosting more than one robot), and that robots share a common chirality. Overall, oblivious deterministic algorithms either need a common coordinate system or cannot form any general pattern. 

To circumvent those impossibility results, the probabilistic path was taken by Yamauchi and Yamashita~\cite{Yamashita2014}. The robots are oblivious, operate in the most general ASYNC model, and can form any general pattern from any general initial configuration (with at least $n\geq5$ robots), without assuming a common coordinate system. However, their approach~\cite{Yamashita2014} makes use of three hypotheses that are not proved to be necessary: \emph{(i)} all robots share a common chirality, \emph{(ii)} a robot may not make an arbitrary long pause while moving (more precisely, it cannot be observed twice at the same position by the same robot in two different Look-Compute-Move cycles while it is moving), and \emph{(iii)} infinitely many random bit are required (a robot requests a point chosen uniformly at random in a continuous segment) anytime access to a random source is performed. While the latter two are of more theoretical interest, the first one is intriguing, as a common chirality was also used extensively in the deterministic case. The following natural open question raises: is a common chirality a necessary requirement for mobile robot \emph{general} gathering ? As the answer is yes in the deterministic~\cite{Flocchini08} case, we concentrate on the probabilistic case.

\paragraph*{Our contribution.}
In this paper, we propose a new probabilistic pattern formation algorithm for oblivious mobile robots that operate in the ASYNC model. Unlike previous work, our algorithm makes no assumptions about the local coordinate systems of robots (they do \emph{not} share a common ``North'' nor a common ``Right''), yet it preserves the ability from any initial configuration that contains at least $7$ robots to form any general pattern (and not just patterns such that $\rho(I)$ divides $\rho(F)$). Besides relieving the chirality assumption, our proposal also gets rid of the previous assumption~\cite{Yamashita2014} that robots do not pause while moving (so, they really are fully asynchronous), and the amount of randomness is kept low -- a single random bit per robot is used per use of the random source -- (\emph{vs.} infinitely many previously~\cite{Yamashita2014}). Our protocol consists in the combination of two phases, a probabilistic leader election phase, and a deterministic pattern formation one. As the deterministic phase does not use chirality, it may be of independent interest in the deterministic context. 

A straightforward extension of our algorithm permits to form patterns with multiplicity points (provided robots are endowed with multiplicity detection), a new feature in the context of pattern formation that we believe is an important feature of our approach.

%Our algorithm releases those three assumptions and allows the pattern to contain points of multiplicity. Actually the only assumption that is not proved to be necessary is that %the initial configuration must not contain multiplicity point.
%%\begin{theorem}
%    The combination of algorithm $\{\RSB,\DPF\}$ forms any pattern $F$ from any initial configuration $I$ that does not contain multiplicity points
%\end{theorem}
%\begin{proof}    
%Lemmas \ref{lem:RSB|Q --> DPF}, \ref{lem:RSB|Qbar --> DPF}, and \ref{lem:RSB <-/- DPF} implies that the combination algorithm $\{\RSB,\DPF\}$ reaches with probability one the %configuration in $\{F\} = stationary(\RSB) \cap stationary(\DPF)$. 
%\end{proof}
%
%The algorithm works without chirality, with only one random bit by robot's activation and even if robots can make a pause during their movement (we do not assume the the strict %progress property \ie, a robot $r$ can see the same robot $r'$ at the same location multiple times even if $r'$ is in the the middle of same Move phase). Moreover the pattern %can contains points of multiplicity.

==> pattern_formation_with_multiplicity_without_detection.tex <==
While the number of visible robot equals the number of destination (so that we know there is no point of multiplicity), we execute phase 3 as usual (avoiding points of multiplicity).
There will be a time when the distance between each robot and its destination will be closer than the half the minimum distance between two destination point. 
When it is the case, robots can start moving toward their destination without caring about points of multiplicity.
When the number of visible robot is lesser than the number of destination, then each robot moves toward the closets destination.


==> proof-figure1.tex <==
%!TEX root = podc.tex


\definecolor{qqwuqq}{rgb}{0.,0.39215686274509803,0.}
\begin{tikzpicture}[line cap=round,line join=round,>=triangle 45,x=1.0cm,y=1.0cm]
\clip(-16.31863394368693,-8.589159525561229) rectangle (16.12932808571511,7.840535534127526);
\draw [shift={(4.999930110658124,-1.0204775771694816)},fill=black,fill opacity=0.15] (0,0) -- (59.13563136375817:1.2342842699265357) arc (59.13563136375817:96.13563136375816:1.2342842699265357) -- cycle;
\draw [shift={(4.375568607115504,4.787633682558667)},fill=black,fill opacity=0.15] (0,0) -- (-109.86436863624185:1.2342842699265357) arc (-109.86436863624185:-83.86436863624185:1.2342842699265357) -- cycle;
\draw [shift={(4.999930110658124,-1.0204775771694816)},fill=black,fill opacity=0.15] (0,0) -- (-0.19554797627085824:1.2342842699265357) arc (-0.19554797627085824:59.13563136375817:1.2342842699265357) -- cycle;
\draw [shift={(4.999930110658124,-1.0204775771694816)},fill=black,fill opacity=0.15] (0,0) -- (-35.426268127565116:1.2342842699265357) arc (-35.426268127565116:-0.19554797627085302:1.2342842699265357) -- cycle;
\draw [domain=-16.31863394368693:16.12932808571511] plot(\x,{(-5.88-0.02*\x)/5.86});
\draw(4.999930110658124,-1.0204775771694816) circle (5.841573734233515cm);
\draw[line width=4.pt,color=qqwuqq,fill=qqwuqq,fill opacity=0.1] (-14.590635965789781,6.359394410215685) -- (-9.65349888608364,6.359394410215685);
\draw [domain=4.999930110658124:16.12932808571511] plot(\x,{(-28.12935766893494--5.014314031034164*\x)/2.9967713444073123});
\draw[line width=4.pt,color=qqwuqq,fill=qqwuqq,fill opacity=0.1] (-14.618064505121483,4.987967443630647) -- (-9.68092742541534,4.987967443630647);
\draw[line width=4.pt,color=qqwuqq,fill=qqwuqq,fill opacity=0.1] (-14.23406495447767,3.3696836230603022) -- (-9.296927874771526,3.3696836230603022);
\draw [domain=-16.31863394368693:4.999930110658124] plot(\x,{(-28.403003459154192--5.808111259728149*\x)/-0.6243615035426204});
\draw (6.227625386971122,0.5171155325634235) node[anchor=north west] {$\tau$};
\draw (5.103055274371389,1.3948287911778476) node[anchor=north west] {$\theta$};
\draw (3.8961995437765538,3.8085402523675147) node[anchor=north west] {$\gamma$};
\draw (8.504194151502286,4.686253510981939) node[anchor=north west] {$r$};
\draw (4.554484487737373,5.947966320240174) node[anchor=north west] {$r'$};
\draw (3.7041997684546484,-0.7445972766948115) node[anchor=north west] {$W(P)$};
\draw (0.5773462846407578,-0.7171687373631107) node[anchor=north west] {$W(P')$};
\draw (4.375568607115504,4.787633682558667)-- (2.2804993221386245,-1.0111962434202686);
\draw (4.999930110658124,-1.0204775771694816)-- (12.,-6.);
\draw (6.419625162293027,-0.7171687373631107) node[anchor=north west] {$\tau'$};
\draw (12.316761118608698,-4.804021097786523) node[anchor=north west] {$p$};
\draw (2.2804993221386245,-1.0111962434202686)-- (12.,-6.);
%\begin{scriptsize}
%\draw[color=black] (-16.099205629033325,-0.49774042270950464) node {$a$};
%\draw [fill=black] (4.999930110658124,-1.0204775771694816) circle (1.5pt);
%\draw [fill=qqwuqq] (-13.82263686450216,6.359394410215685) circle (2.5pt);
%\draw[color=qqwuqq] (-13.301494617199843,6.990250814844803) node {$\tau = 28\textrm{\degre}$};
%\draw [fill=black] (7.996701455065437,3.9938364538646827) circle (1.5pt);
%\draw [fill=qqwuqq] (-10.558640684029765,4.987967443630647) circle (2.5pt);
%\draw[color=qqwuqq] (-9.872927200737244,5.6188238482597646) node {$\gamma = 37\textrm{\degre}$};
%\draw [fill=qqwuqq] (-13.027209223882835,3.3696836230603022) circle (2.5pt);
%\draw[color=qqwuqq] (-12.341495740590316,4.00054002768942) node {$\delta = 11\textrm{\degre}$};
%\draw [fill=black] (4.375568607115504,4.787633682558667) circle (1.5pt);
%\draw [fill=black] (2.2804993221386245,-1.0111962434202686) circle (1.5pt);
%\draw [fill=black] (18.,1.0580163140195609) circle (1.5pt);
%\draw[color=black] (17.63789774895865,1.4496858698412491) node {$H$};
%\draw [fill=black] (12.,-6.) circle (1.5pt);
%\end{scriptsize}
\end{tikzpicture}
